DefectHunter: A Novel LLM-Driven Boosted-Conformer-based Code Vulnerability Detection Mechanism

One of the most pressing threats to computing systems is software vulnerabilities, which can compromise both hardware and software components. Existing methods for vulnerability detection remain suboptimal. Traditional techniques are both time-consuming and labor-intensive, while machine-learning-based approaches often underperform when applied to complex datasets, due to their inability to capture high-dimensional relationships. Previous deep-learning strategies also fall short in capturing sufficient feature information. Although self-attention mechanisms can process information over long distances, they fail to capture structural information. In this paper, we introduce DefectHunter, an innovative model for vulnerability identification that employs the Conformer mechanism. This mechanism fuses self-attention with convolutional networks to capture both local, position-wise features and global, content-based interactions. Furthermore, we optimize the self-attention mechanisms to mitigate the issue of excessive attention heads introducing extraneous noise by adjusting the denominator. We evaluated DefectHunter against ten baseline methods using six industrial and two highly complex datasets. On the QEMU dataset, DefectHunter exhibited a 20.62\% improvement in accuracy over Pongo-70B, and for the CWE-754 dataset, its accuracy was 14.64\% higher. To investigate how DefectHunter comprehends vulnerabilities, we conducted a case study, which revealed that our model effectively understands the mechanisms underlying vulnerabilities.

==> discuss.tex <==
%Although it is shown in the evaluation part that our proposed approach and implementation can have a sound effect against dangerous smart home apps, however, as aforementioned, our approach cannot defend against open-port based attacks due to the reasons illustrated in Section~\ref{sec:background}. Fortunately, there are multiple alternatives that may have the potential to mitigate these attacks. 
%\begin{itemize}
%\item \textbf{Inhibiting Dictionary Attacks.} Dictionary attacks is the first step that Mirai took to compromise IoT devices~\cite{mirai}. Therefore, inhibiting dictionary attacks may effectively hinder Mirai and similar botnets exploiting weak credentials. Currently, multiple solutions have been proposed to inhibit the dictionary attacks from different aspects~\cite{bontrager2018}\cite{2016wuhiera}. Yet, these solutions are mainly designed for general-purpose computing systems. Whether or not they can be migrated to the embedded systems needs to be further scrutinized.
%
%\item \textbf{Code-Level Vulnerability Discovery.} Sophisticated botnets (e.g., IoTReaper) exploits a number of zero-day vulnerabilities to compromise IoT devices~\cite{greenberg2017reaper}. Therefore, code-level bug searching techniques may serve as ideal solutions to mitigate the zero-day based open-port attacks~\cite{shoshitaishvili2015firmalice}\cite{muench2018you}\cite{Zheng2017usenix}.
%
%\item \textbf{Hardware-Assisted Approaches.} Some zero-day vulnerabilities may be too complicated to be uncovered using merely the static code-level analysis. In this case, leveraging hardware as an assistant to isolate sensitive information/codes from the insensitive ones can constrain the damages brought by the zero-day vulnerabilities~\cite{Frassetto2018imix}\cite{weiser2019timber}. 
%\end{itemize}
